GCRE-GPT: A Generative Model for Comparative Relation Extraction

Given comparative text, comparative relation extraction aims to extract two targets (\eg two cameras) in comparison and the aspect they are compared for (\eg image quality). The extracted comparative relations form the basis of further opinion analysis.Existing solutions formulate this task as a sequence labeling task, to extract targets and aspects. However, they cannot directly extract comparative relation(s) from text. In this paper, we show that comparative relations can be directly extracted with high accuracy, by generative model. Based on GPT-2, we propose a Generation-based Comparative Relation Extractor (GCRE-GPT). Experiment results show that \modelname achieves state-of-the-art accuracy on two datasets.

==> tables/task_representation.tex <==
\begin{table}
  \centering
  \caption{The expression of relation for existing methods.}
 \scriptsize
  \caption{Different relation description in different model and predicate refers to the word or phrase that is used to express the comparison}
  %\scalebox{0.9}{
    \begin{tabular}{l|l}
    \toprule
    Method &  Expression of Relation \\
    \midrule
   LSR~\cite{DBLP:conf/aaai/JindalL06}   & (predicate,\{aspect\}, \{subject\}, \{object\})  \\
    SRL~\cite{DBLP:conf/emnlp/KesslerK13}   & (predicate, entity+, entity-, aspect)   \\
    CRF~\cite{DBLP:journals/comsis/WangXWHL17}   & (subject, object, aspect, predicate)   \\
    LSTM~\cite{DBLP:conf/cikm/AroraAGP17}  & (subject, object, aspect, predicate)        \\
    BERT-CRF~\cite{DBLP:conf/emnlp/LiuXY21} & (subject, object,aspect, predicate) \\
    \bottomrule
    \end{tabular}%%}
  \label{tab:task_representation}%
\end{table}%

